Tube-Based Zonotopic Data-Driven Predictive Control

We present a novel tube-based data-driven predictive control method for linear systems affected by a bounded addictive disturbance. Our method leverages recent results in the reachability analysis of unknown linear systems to formulate and solve a robust tube-based predictive control problem. More precisely, our approach consists in deriving, from the collected data, a zonotope that includes the true state error set. We show how to guarantee the stability of the resulting error zonotope, which can be exploited to increase the computational efficiency of existing zonotopic data-driven MPC formulations. Results on a double-integrator affected by strong adversarial noise demonstrate the effectiveness of the proposed control approach.

==> _ignore/other.tex <==
\\\\
\newpage
\noindent \textbf{Computing $(\Delta A,\Delta B, K)$.} To solve the optimization problem in \Cref{problem:robust_tz-ddpc} we need few more ingredients, i.e. the knowledge of $(\Delta A,\Delta B)$, or, at least, knowledge of an upper-bound $(\|\Delta A\|,\|\Delta B\|)$ that can be used to over approximate the zonotope $\zonotope_{e,t}$ of the error signal. However, even with the knowledge of $(\|\Delta A\|,\|\Delta B\|)$ we may not be able to guarantee the stability of $\closedloopA + \Delta A + \Delta B K$ unless one neglects the disturbance term $\Delta A + \Delta B K$ and computes $K$ only on the basis of $(A_0,B_0)$. Nonetheless, we introduce the following lemma that shows how to bound the error zonotope.

Using this lemma, and an estimate of $(\|\Delta A\|, \|\Delta B\|)$, we can  find some matrices $\tilde A,\tilde B$ that are full-rank to be used to over-approximate $\zonotope{e,t}$:
\begin{equation}
    \zonotope{e,t} \subset E Z_{e,t-1} + \alpha_{\Delta A,\tilde A}\tilde A \langle \bar x_t, I_n\rangle\ + \alpha_{\Delta B,\tilde B}\tilde BK \langle \bar u_t, I_m \rangle   + \zonotope{w},
\end{equation}
with $E = A_0+B_0K+\alpha_{\Delta A,\tilde A}\tilde A + \alpha_{\Delta B,\tilde B} \tilde B K$.
\\\\




We focus on solving the robust problem in \Cref{problem:p_x} using data-driven control methods. Inspired by the zonotope based approach in \cite{alanwar2022robust}, we propose \textsc{SZ-DDPC}, a scenario-based data-driven approach, to robustly solve the optimization problem $\mathcal{P}_N(x_t)$.

Solving min-max problems is notoriously difficult, and  solving directly the problem in \Cref{problem:p_x} may be computationally prohibitive. In contrast to classical min-max MPC formulations \cite{lofberg2003minimax}, here we consider that also the pair $(A,B)$ is uncertain, which increases the difficulty of the problem. In \cite{alanwar2022robust} the authors consider a robust control problem that exploits data-driven reachability analysis, and propose \textsc{ZPC}. However, their formulation  is computationally complex even when the user introduces over-approximation of the zonotopes, and the algorithm poorly scales over the horizon $N$, an important property of any receding-horizon algorithm. Consequently,  the resulting control policy of \textsc{ZPC} is usually myopic, which may limit the stability guarantees of \textsc{ZPC}.
\subsubsection{Solving \cref{problem:p_x}}

Instead, we propose a tube-based approach that takes advantage of the reachability analysis conducted in \cite{alanwar2021data}.

In tube-based MPC the control law is given by $\mu_N^\star(x_t) = u_{1|t}^\star(x_t) + K(x_t-\bar x_t)$, where $u_{1|t}^\star(x_t) $ is the first variable of the optimal control sequence yield by MPC, and $\bar x_t$ describes the nominal dynamics of the model. $K$ is chosen so that $e_{t+1}=(A+BK)e_t +w_k, e_t = x_t-\bar x_t$ is asymptotically stable, which guarantees that $e_t \in \zonotope{w}\oplus (A+BK) \zonotope{w} \oplus \cdots \oplus (A+BK)^{t-1}\zonotope{w} \subset \frac{1}{1-\rho(A+BK)}\zonotope{w}$. In our case $(A,B)$ is not known, which leads to two problems: (1) how to design $K$; (2) how to compute the predictive dynamics of the nominal model $\bar x_t$.

We split our algorithm into two phases: in the first one, which can be conducted in the offline learning phase, we design $K$ such that $A+BK$ is stable against the worst possible pair $(A,B)\in \constrainedmatrixzonotope{\data}$. Formally, let

\begin{equation}
    
\end{equation}


However, taking inspiration from \textsc{ZPC}, and robust MPC,  we formulate the following optimization problem:
\begin{equation}\label{problem:p_x_2}
\begin{aligned}
\bar{\mathcal{P}}_N(x_t): &\min_{u_{1|t},\dots,u_{N|t}} \max_{(A,B)\in \constrainedmatrixzonotope{\data}}\quad  \sum_{k=1}^{N} \ell_k(x_{k|t},u_{k|t})\\
\textrm{s.t.} \quad 
&x_{k+1|t}=Ax_{k|t}+Bu_{k|t}\quad x_{1|t}=x_t,\\
& x_{k+1|t} +\zonotope{S_{k+1|t}} \subseteq  {\zonotope{x}},\\
& \zonotope{S_{k+1|t}} = \zonotope{S_{k|t}} \oplus A^{k-1}\zonotope{w}, \quad \zonotope{S_{1|t}} = \emptyset\\
& u_{k|t} \in \zonotope{u},\quad k=1,\dots, N
\end{aligned}
\end{equation}
The formulation in \Cref{problem:p_x_2} follows from the intuition that for any matrix $A$ the contribution of the noise at time $k+1$ is given by $\zonotope{S_{k+1|t}} =\zonotope{w} \oplus A\zonotope{w}\oplus \cdots \oplus A^{k-1}\zonotope{w}$. Consequently,  we bound the state $x_{k+1|t}$ in the optimization problem so that the set $x_{k+1} +\zonotope{S_{k+1|t}} $ is contained in the state constraint zonotope $\zonotope{x}$ for all $k=1,\dots,N$. If the initial point $x_t$ is contained in a set $\mathcal{X} \supseteq \zonotope{x}$, this guarantees the feasibility of the problem.

\begin{equation}\label{problem:p_x_2}
\begin{aligned}
\bar{\mathcal{P}}_N(x_t): &\min_{v_{1|t},\dots,v_{N|t}} \quad  \sum_{k=1}^{N} \ell_k(\bar x_{k|t},u_{k|t})\\
\textrm{s.t.} \quad 
&\bar x_{k+1|t}=A_0\bar x_{k|t}+B_0 v_{k|t}\quad \bar x_{1|t}=x_t,\\
& e_{k+1|t} \in \\
& \bar x_{k+1|t} \in \zonotope{x} \ominus \zonotope{e,k},\\
& \zonotope{e,k+1} = (A_{cl} +\Delta A) \zonotope{e,k}+\Delta A \bar x_{k|t} + \Delta B u_{k,t}, \quad \zonotope{S_{1|t}} = \emptyset\\
& v_{k|t} \in \zonotope{u} \ominus 
\zonotope{u_{\text{tube}},k},\quad k=1,\dots, N
\end{aligned}
\end{equation}

\begin{lemma}[Region of attraction]
Assume $\bar{\mathcal{P}}_N(x_0)$ is feasible over an horizon $N$ for any initial point $x_1 \in \mathcal{X}$, with $\zonotope{x} \subseteq \mathcal{X}$. If $x_{N+1|1} +\zonotope{S_{N+1|1}} \subseteq \zonotope{x} $, then the optimization in \Cref{problem:p_x_2} is guaranteed to be feasible at all times $t>0$ and $\mathcal{X}$ is a region of attraction.
\end{lemma}
\begin{proof}
The proof follows from a simple recursive feasibility argument.
\end{proof}


\begin{lemma}
Let $(A^\star,B^\star)$ be the true pair of the system in \Cref{eq:system}.
\end{lemma}
\begin{proof}
For simplicity, let $t=1$, and denote the true state of the system by $x_k$ , then $x_{k+1}=A^\star x_k + B^\star u_k^\star + w_k$.
Define by $e_k = x_k -x_{k|t}$ the error.
\end{proof}


\begin{lemma}
For any Schur matrix $A$ the set induced by the zonotope $\lim_{k\to\infty} \zonotope{S_{k+1|t}} $ exists, and is bounded.
\end{lemma}
\begin{proof}
The proof simply follows from the fact that $\lim_{k\to\infty}\zonotope{S_{k+1|t}} = \lim_{k\to\infty} \zonotope{w} \oplus A\zonotope{w}\oplus \cdots \oplus A^{k-1} \zonotope{w} \subseteq \lim_{k\to\infty} \zonotope{w}\sum_{n=1}^k \rho(a)^{n-1} =   \frac{1}{1-\rho(a)}\zonotope{w}$.
\end{proof}


 Solving directly the problem in \ref{problem_robust_rhc} may be computationally prohibitive. Motivated by this reason, we resort to using a randomized approach to solve the RHC problem in \ref{problem_rhc}. First, for some $\mathcal{S}\in \mathcal{T}$, let us define $\mathcal{L}_{t_0,N}(& u_0,\dots,u_{N-1};\mathcal{S})$, which represents  the cost of applying a specific input sequence $(u_0,\dots, u_{N-1})$ starting at $t_0$ to a specific system $\mathcal{S}$:



One of the difficulty in \Cref{problem:p_x} arises from the fact that 

use results from uncertain convex programming \cite{calafiore2005uncertain,campi2008exact} and  data-driven reachability analysis \cite{alanwar2021data}. 

We start by 

In the following, we consider a robust data-driven formulation of \Cref{problem_rhc}.


Therefore, following the approach used in \cite{alanwar2021data}, it is possible to construct a constrained noise zonotope $\constrainedzonotope{w}$ that is consistent with the data, defined by the following set
\begin{equation}
    \matrixzonotope{w} = \{W_- \in \
\end{equation}

We now recall the following result from \cite{alanwar2021data}, which states that $\Sigma_\mathcal{D}$ can be represented in terms of a constrained matrix zonotope $\matrixzonotope{\mathcal{D}}$ that is an over-approximation of $\Sigma_\mathcal{D}$.
\begin{lemma}
Given input-state trajectory
\end{lemma}


We make the following assumption of stabilizability, so that the uncontrollable space of the system is naturally stable.
\begin{assumption}
We assume that $\Sigma \subseteq \Sigma_{\text{stab}}=\{(A,B): (A,B) \text{ is stabilizable}\}.$
\end{assumption}


We consider the  receding horizon control (RHC) problem for an unknown system $\mathcal{S}$, either of type (\SMEAS) or (\SIO). In general, the classical RHC formulation can be defined as follows 
\begin{equation}\label{problem_rhc}
\begin{aligned}
\min_u \quad & \sum_{k=0}^{N-1} \ell(y_{t_0+k+1|t}, u_{t_0+k+1|t}) \\
\textrm{s.t.} \quad 
& y_{t_0+k+1|t} \text{ generated according to } \mathcal{S}\\
& y_{t_0+k+1|t}\in \zonotope{y},u_{t_0+k|t}\in\zonotope{u} \quad k\in[N-1]
\end{aligned}
\end{equation}
where $N$ is the horizon length,  $\ell: \mathbb{R}^n\times\mathbb{R}^m\to [0,\infty)$ is a convex loss function, $\zonotope{y}$ is the output constraint zonotope, $\zonotope{u}$ is the input constraint zonotope, and  $y(t_0)$ is the initial point. In the following, we consider a robust data-driven formulation of \Cref{problem_rhc}.



As previously mentioned, Zonotopes have been investigated for  data-driven predictive control in \cite{alanwar2022robust}, where the authors proposed \textsc{ZPC}: Zonotopic Data-Driven Control. However, the formulation in \cite{alanwar2022robust} poorly scales over the horizon $N$. The authors introduce approximations, which ease the computational burden of  \textsc{ZPC}. In particular, they over-approximate the system matrix zonotope by an interval matrix, and constrain the output $y(k)$ by considering the interval matrix of the reachable set at time $k$. As a consequence, the control policy computed by \textsc{ZPC} is myopic, and the introduced over-approximations may hinder the robustness of \textsc{ZPC}.

\noindent Instead, in this work we consider the following robust formulation of the RHC problem:
\begin{equation}\label{problem_robust_rhc}
\begin{aligned}
\min_{u_{0},\dots,u_{N-1}}& \max_{\mathcal{S}\in \mathcal{T}}\quad  \sum_{k=0}^{N-1} \ell(y_{k+1}, u_k) \\
\textrm{s.t.} \quad 
&y_{k+1} \text{ generated according to } \mathcal{S}, y_0=y(t_0)\\
& y_{k+1}\in \zonotope{y},u_{k}\in\zonotope{u} \quad k\in[N-1]
\end{aligned}
\end{equation}
for some set of systems $\mathcal{T}$, which contains the true system $\mathcal{S}^\star$, and $\mathcal{T}$ may be a continuous set containing an infinite number of instances. 


\subsection{Offline phase: data-collection}

\begin{lemma}[Regularization of LTI Reachability] Consider an LTI system of the type
\begin{equation}
    x_{t+1} = Ax_t + Bu_t +w_t, \quad y_t = \bar x_t +v_t
\end{equation}
where $\bar x_t \in \mathbb{R}^{\bar n}$ is the observable part of $x_t$, i.e., $x = \begin{bmatrix}\bar x& \tilde x\end{bmatrix}^\top$ and $\tilde x\in \mathbb{R}^{n-\bar n}$ is the unobservable part. Assume 
\end{lemma}
\begin{proof}
Similarly to \cite{alanwar2021data,de2019formulas}, given input-output trajectories $\mathcal{D}=(U_{-}, Y)$, we can write
\begin{align*}
   Y_+ -V_+&= A_{11}(Y_- - V_-) + A_{12} \tilde X_- + B_1 U_- + W_{1,-},\\
   \tilde X_+&= A_{21} (Y_- - V_-) + A_{22} \tilde X_- + B_2U_- + W_{2,-}.
\end{align*}
Rearranging the terms, leads to
\begin{align*}
   Y_+ -(V_+- A_{11}V_-)-W_{1,-}&= A_{11}Y_- + A_{12} \tilde X_- + B_1 U_- ,\\
   \tilde X_+ - A_{22} \tilde X_- -  W_{2,-}&= A_{21} (Y_- - V_-) + B_2U_- .\\
\end{align*}
Then, using lemma 1 in \cite{alanwar2021data}
\begin{align*}
    \begin{bmatrix}A_{11} &B_1 \end{bmatrix} = (Y_+ - \matrixzonotope{Av}-\matrixzonotope{w_1}-A_{12}\matrixzonotope{\tilde x})\begin{bmatrix}Y_- \\ U_-\end{bmatrix}^\dagger
\end{align*}
Let $a_{i,j}$ be known bounds on $A_{i,j}$ such that $\|A_{i,j}\| \leq a_{i,j}$, then
\[
\| \tilde x_+\| \leq a_{22} + \bar w_2 + a_12 \|y_-\| + b_2 \|u_-\|
\]
\end{proof}



\subsubsection{Linear Systems with Process Noise}

\subsubsection{Input-Output Data Linear Systems with Process Noise}
\subsection{Online control phase}
In the previous section, we have seen how to construct $\mathcal{T}$, a set of systems that is consistent with the data $D$ collected from the true system $\mathcal{S}^\star$. 

 Solving directly the problem in \ref{problem_robust_rhc} may be computationally prohibitive. Motivated by this reason, we resort to using a randomized approach to solve the RHC problem in \ref{problem_rhc}. First, for some $\mathcal{S}\in \mathcal{T}$, let us define $\mathcal{L}_{t_0,N}(& u_0,\dots,u_{N-1};\mathcal{S})$, which represents  the cost of applying a specific input sequence $(u_0,\dots, u_{N-1})$ starting at $t_0$ to a specific system $\mathcal{S}$:
 \begin{equation}
 \begin{aligned}
     \mathcal{L}_{t_0,N}(& u_0,\dots,u_{N-1};\mathcal{S}) = \Bigg\{\sum_{k=t_0}^{t_0+N-1} \ell(y_{k+1|t}, u_{k}): \\
     & y_{k+1|t} \text{ generated according to } \mathcal{S}, y_{k+1|t}\in \zonotope{y} \Bigg\}
\end{aligned}.
 \end{equation}
 Now, define a probability measure $\mathbb{P}$ over $\mathcal{T}$, which can be interpreted in different ways: it can represent the level of certainty about the true $\mathcal{S}^\star$, or the relative importance we attribute to different systems $\mathcal{S}\in \mathcal{T}$. 
 Ultimately, since we have access to $\mathcal{T}$, we can o define the corresponding randomized convex program by sampling $L$ i.i.d. instances of systems $\mathcal{S}^{(1)}, \mathcal{S}^{(L)}$. Then, the sampled convex program derived from \ref{problem_robust_rhc} is
 
\begin{equation}\label{problem_sampled_robust_rhc}
\begin{aligned}
\text{SCP : }&\min_{u_0,\dots,u_{N-1}, \nu} \quad  \nu \\
\textrm{s.t.} \quad 
& \mathcal{L}_{t_0,N}(u_0,\dots,u_{N-1};\mathcal{S}^{(i)})-\nu\leq 0,\quad i\in [L]\\
& u_{k}\in\zonotope{u} \quad k\in[N-1]
\end{aligned}
\end{equation}




